Dynamic Accountable Storage: An Efficient Protocol for Real-time Cloud Storage Auditing

Ateniese, Goodrich, Lekakis, Papamanthou, Paraskevas, and Tamassia introduced the Accountable Storage protocol, which is a way for a client to outsource their data to a cloud storage provider while allowing the client to periodically perform accountability challenges. An accountability challenge efficiently recovers any pieces of data the server has lost or corrupted, allowing the client to extract the original copies of the damaged or lost data objects. A severe limitation of the prior accountable storage scheme of Ateniese et al., however, is that it is not fully dynamic. That is, it does not allow a client to freely insert and delete data from the outsourced data set after initializing the protocol, giving the protocol limited practical use in the real world. In this paper, we present Dynamic Accountable Storage, which is an efficient way for a client to periodically audit their cloud storage while also supporting insert and delete operations on the data set. To do so, we introduce a data structure, the IBLT tree, which allows either the server or the client to reconstruct data the server has lost or corrupted in a space-efficient way.

==> sections/abstract.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Dynamic Accountable Storage [Make more cloud-y]}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.

\author{Vinesh 
Sridhar}
\affiliation{%
  \institution{The University of California, Irvine}
  \city{Irvine}
  \country{USA}}
\email{vineshs1@uci.edu}


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Goodrich et al.}
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%


%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Do, Not, Us, This, Code, Put, the, Correct, Terms, for,
  Your, Paper}

\received{20 February 2007}
\received[revised]{12 March 2009}
\received[accepted]{5 June 2009}


%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
  A clear and well-documented \LaTeX\ document is presented as an
  article formatted for publication by ACM in a conference proceedings
  or journal publication. Based on the ``acmart'' document class, this
  article presents and explains many of the common variations, as well
  as many of the formatting elements an author may use in the
  preparation of the documentation of their work.
\end{abstract}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle


==> sections/dynamic-accountable-storage-model.tex <==
\section{Dynamic Accountable Storage Model}\label{sec:model}

% \subsection{Overview}\label{sec:overview}

% % Throughout the paper, we discuss the protocol in terms of two parties: the \emph{client}, who owns some data but has limited resources to manage it, and the \emph{server}, the entity to which the client is outsourcing her data. 

% \subsubsection{Trust Model.}
% As we described above, if the client has already chosen the server to store her data, the she trusts the server not to maliciously tamper her data. Furthermore, because the client can switch to another provider if service is poor, the server has a monetary incentive to do its best to recover the client's data in any way it can to avoid an SLA violation. 

% \subsubsection{Additions to the Accountable Storage Protocol.}
% \vinesh{Mention something about change in security requirements, as a result no PDP needed??}



% \subsubsection{Protocol.}

% The client begins with her data padded into blocks $B = \{b_1, ..., b_n\}$ of equal size in local storage. Realistically, to be able to access her data, the client must maintain a store of small keys $K = \{k_1, ..., k_n\}$ that correspond to each block. We assume each block has a unique key. 

% The client chooses an acceptable $\delta$ for her use case. Here, $\delta$ determines the level of security she wishes to have. A larger $\delta$ means she can recover more corrupted blocks, but requires more local storage. Generally, if accountability challenges happen periodically and the cloud storage host is reasonably trusted, we assume $\delta$ is very small. 

% The client then generates a data structure called an Invertible Bloom Lookup Table (described in Section~\ref{sec:IBLT-def}) as well as a set of cryptographic tags $\Phi$ to the server. As described above, the tags can be batched together to save communication complexity in a proof. 

% After this, the client sends $pk, B,$ and her set of tags $\Phi$ to the server. Now the client is free to delete her blocks and tags. However, the client keeps the IBLT $T_B$.

% Now the client can request blocks by sending the server a set of keys $K'$ such that $|K'| < \delta$. Let $B'$ be the blocks that correspond to the keys $K'$. The server can construct an IBLT $T_K$ of the blocks $B - B'$ and send it to the client along with the corresponding tags. Then the client can perform an IBLT subtraction operation to produce an IBLT with just the blocks in $B'$. With high probability, the client can recover these blocks. 
% In our implementation, we incorporate the index of a block $b_i$ into its tag $\phi_i$. This presents a problem if we allowed arbitrary insertion and deletion: because of shifting indices, the client may have to recompute $O(n)$ tags. Thus, we require that insertions only append to the end of the database and that deletions are replaced by the last element, ensuring $O(1)$ tag computations per update. If the client desires a logical ordering to her data, a separate key-value store can be maintained by the server.

% During a request, the server is able to efficiently detect whether it has correctly maintained its data using its IBLT tree. If it finds a corruption, it executes a restore operation that allows it to recover up to $\delta$ lost elements under certain conditions \vinesh{what conditions?}.

% In addition, the client can issue an accountability challenge to the server. This prompts the server to respond with an IBLT $T_K$ containing {\it all} the blocks the server has. When the client receives $\mathcal{V}$, she can take the difference $T_B - T_K$ to produce an IBLT $T_L$ containing just the $\leq \delta$ corrupted or missing blocks. From here she can extract both the $\delta$ correct blocks as well as their corrupted counterparts. See the original Accountable Storage paper for a detailed description of this process \cite{ateniese2017accountable}. She can then easily compute the damage $d$ using a metric such as the Hamming Distance \cite{hamming1950error}. 

% In this work, we consider the notion of \emph{incremental trust}. Any time the client attempts to change its state, we require the server to send proofs alongside any information the client needs verifying that data's validity. This ensures that the client has an accurate representation of its own data. 

% Once a change is made to the state, we assume that the server will not try to tamper with that state and trick the client. We believe that this is a realistic model in the context of commercial cloud services, wherein the server may make errors in transactions with the client, but does not do so maliciously. 

% \subsection{Challenges in Making the Scheme Dynamic}
% \vinesh{retool somehow.}
% There are two key challenges in making this scheme dynamic. 
% In addition, the communication efficiency of accountability challenges relies on using homomorphic tags. In our implementation, tags are bound to the index of a given block. Thus, having arbitrary insertion or deletion would cause the client to have to recreate $O(n)$ tags. Instead, we apply a classic idea in maintaining unsorted data: we only allow insertions at the end of the structure and any deletion has the deleted element be replaced by the last element. Thus, the client is only required to recreate $O(1)$ tags per operation. If the client wishes to have a logical ordering to their data, a separate key-value pair structure can be maintained by the server. 

% \subsection{Model of the Protocol}

\vinesh{Intro paragraph, benign model. Correctness. Combine with section 5. }

\begin{definition}[Dynamic $\delta$-AS scheme]\label{def:DAS}
    A dynamic $\delta$-AS scheme has the following polynomial-time functions:
\begin{enumerate}

\item $(pk, sk, T, state, I) \leftarrow Setup(B, K, \delta, 1^\tau, \beta)$. Takes as input the client's set of blocks and keys $(B, K)$, the parameter $\delta$, the security parameter $\tau$, and the server parameter $\beta$. Returns a public and secret key $(pk, sk)$, a set of tags $T$, the client state, and the server's zip-IBLT tree $I$. 

\item $(state') \leftarrow Insert(k, b, state)$. Takes the new key-block pair and the client's state. Inserts the block at the client and the server and returns the client's new state.

\item $(state') \leftarrow Remove(k, state)$. Takes a key held by the client and the client's state. Deletes the corresponding block from the client and server and returns the client's new state.

\item $\{B', \texttt{reject}\} \leftarrow ClientAudit(K', state)$. Takes a set of keys $K'$ the client wishes to audit and the client's state. Returns the corresponding correct blocks or \texttt{reject}, if the blocks could not be recovered correctly. 

\item $\{B', \texttt{failure}\} \leftarrow ServerAudit(K', I)$. Takes a set of keys the server wishes to audit and the server's state. Returns the corresponding correct blocks or \texttt{failure}, if the blocks could not be recovered correctly. 

\item $\{\mathcal L, \texttt{reject}\}\leftarrow AccountabilityChallenge(state)$. Takes the client's state. Performs an audit of the entire data base. The client returns a set $\mathcal L$ of blocks that the server has corrupted, or \texttt{reject} if the client could not recover the corrupted blocks. 

\end{enumerate}
    
    % \begin{enumerate}
    %     \item $(pk, sk, state, T_1, ..., T_n) \leftarrow Setup(B, K, \delta, 1^\tau)$ takes the set of blocks and keys, the parameter $\delta$, and the security parameter $\tau$. It returns a public key $pk$, secret key $sk$, tags $T_1, ..., T_n$, and client state.
    %     % \item $(pk, sk) \leftarrow KeyGen(1^\tau)$ takes the security parameter $\tau$ and returns a pair of of matching public and secret keys. It is run by the client at the beginning of execution.
    %     % \item $state \leftarrow GenState(pk, B, \delta)$ takes the public key, the client's initial set of blocks, and the AS parameter $\delta$. It is run by the client and returns the client's initial state.
    %     % \item $\phi \leftarrow GenTag(sk, b, i)$ takes the secret key, a block, and its index. The client runs it to compute a cryptographic tag $\phi$ corresponding with the block. 
    %     % \item $\mathcal T \leftarrow GenAuthStruct(pk, B)$ is run by the server. It takes the initial set of blocks and creates a data structure that will be used to prove that it maintains the client's data.
    %     % \item $\{(b_i, P), \texttt{failure}\} \leftarrow RetrieveBlock(i, T)$ is run by the server and returns the block at index $i$ held by the server. It uses its authentication structure $T$ to compile a proof of correctness $P$.
    %     % \item $state' \leftarrow PrepInsert(pk, state, b')$ takes the public key, the client's current state, and the new block $b'$. It is run by the client and returns the client's updated state.
    %     % \item $state' \leftarrow PrepReplace(pk, state, b', i)$ takes the public key, the client's current state, the new block $b'$, and the index to replace at. It is run by the client and returns the client's updated state.
    %     % \item $state' \leftarrow PrepDelete(pk, state, i)$ takes the public key, the client's current state, and the index to delete at. It is run by the client and returns the client's updated state.
    %     \item $state' \leftarrow PrepUpdate(pk, state, b', i)$ takes the public key, the client's current state, the new block $b'$ ($\bot$ if a deletion), and the index to update at (always $n$ for an insertion). It is run by the client and returns the client's updated state.
    %     \item $(B', P) \leftarrow GenUpdate(B, req, i, b')$ takes an ordered collection $B$ of blocks, an update request, the index the update affects, and the new block ($\bot$ if $req$ is a deletion). This function is run by the server. It returns an updated set of blocks and a proof that it sends to the client.
    %     \item $\{\emph{\texttt{reject}}, R'\} \leftarrow CheckProof(R, P)$ takes the root of the authentication structure the client maintains and the proof $P$ sent by the server. It is run by the client and either outputs a rejection of the proof or the new root of the authentication structure. 
    %     % \item $chal \leftarrow GenChal(1^\tau)$ takes the security parameter. It is run by the client and returns an accountable storage challenge to be sent to the server.
    %     \item $\mathcal V \leftarrow GenAccountabilityProof(pk, B, \Sigma, chal)$ takes the public key, an ordered collection of $B$ blocks, metadata $\Sigma$, and the client's challenge $chal$. It is run by the server and returns a proof of accountability $\mathcal{V}$ for $B$.
    %     \item $\{\emph{\texttt{reject}}, \mathcal L\} \leftarrow CheckAccountabilityProof(pk, sk, state, \mathcal V, chal, R)$ takes the public and secret keys, the client's current state, the proof of accountability $\mathcal V$ and the challenge $chal$. It is run by the client and returns either a rejection of the proof, or with high probability, a set of blocks $\mathcal L$ that represent the number of corrupted blocks the server held. 
    % \end{enumerate}
\end{definition}

% Intuitively, to be correct, the client's current state must always match the set of data that it believes the server holds. Any insertion, deletion, and replacement that affects $B$ held by the server should result in the same operation being done on the client's $T_B$. In addition, during a proof of accountability, if the server acts honestly, we want to guarantee that the client actually recovers and outputs the blocks $\mathcal L$ that the server corrupted.

\begin{definition}[Dynamic $\delta$-AS scheme correctness]\label{def:DAS-correctness}

Let $\mathcal P$ be a dynamic $\delta$-AS scheme as defined in Definition~\ref{def:DAS}. $\mathcal P$ is correct if 
for all $\tau \in \mathbb{Z}$,
for all $\{pk, sk\}$, tags $t_b$, and states output by $Setup$,
and for all changes to $state$ made by $Insert$ or $Remove$, the following statements hold:

% Let $K'$, $B'$, $T'$ be the set of keys, blocks, and tags held by the server if the server processed all changes correctly.

\begin{enumerate}
    \item For all sets $K^* \subset K$ such that $|K^*| \leq \delta$ input into $ClientAudit$ and $ServerAudit$, the probability that the corresponding blocks $B'$ are output happens with probability $1 - 1/\text{poly}(\delta)$. 
    \item For all sets of corrupted blocks $\mathcal L \subset B'$ such that $|\mathcal L| < \delta$, $AccountabilityChallenge$ outputs $\mathcal L$ with probability $1 - 1/\text{poly}(\delta)$.

\end{enumerate}


\end{definition}
% First we will provide an informal description: in this protocol, the adversary has the incentive to forge a proof that it has maintained all of the client's blocks properly in order to avoid the penalty. Thus, to be secure, we must guarantee that if the adversary issues a valid proof for some block $b_i$, that the adversary must have $b_i$. However, note that our notion of incremental trust discussed in Section~\ref{sec:adversary-model} prevents the server from sending a previously valid block that was deleted or replaced. 
% Because our scheme is dynamic, the client must request blocks from the server---to delete or replace them in their IBLT for example. Thus we also require that, when the client asks for block $b_i$ and the server is able to issue a valid proof along with some block $b_i'$, that $b_i = b_i'$. 

% We describe the security of the protocol in terms of a game between a challenger and an adversary that combines aspects of the Data Possession Game by Erway {\it et al.} \cite{erwayDynamicProvableData2008} and the original Accountable Storage game \cite{ateniese2017accountable}. The adversary's goal is to forge a proof of accountability from which $\mathcal C$ recovers a set $\mathcal L$ of lost blocks such that either (1) $\mathcal L$ is too large, (2) $\mathcal L$ is not a subset of the original blocks, or (3) $\mathcal A$ does not maintain all of the remaining $B - \mathcal L$ blocks. 

\begin{theorem}[Dynamic $\delta$-AS scheme]
    For all $\delta, \beta < n$, there exists a scheme such that:
    (1) it is correct according to Definition~\ref{def:DAS-correctness}; 
    % (2) it is secure in the random oracle model based on the RSA assumption and according to Definition~\ref{def:DAS-security}; 
    (2) The accountability proof has size $O(\delta)$. Its computation at the server takes $O(\beta)$ time, and verification at the client takes $O(\delta\log n)$ time; 
    (3) The space at the client is $O(\delta)$; 
    (4) The space at the server is $O(n + \delta n/\beta)$; 
    (5) Inserting an element takes $O(1)$ time at the client and $O(\log n)$ time at the server; 
    (6) Deleting an element takes $O(\delta\log n)$ time at the client and $O(\beta + \log n)$ time at the server. 
\end{theorem}

\vinesh{Is there a faster way to delete for client? Maybe we have the server audit themselves to regenerate the block and then just send to client?}
\ryuto{I think you could make it constant for the client. Will need to talk about it.}

% \begin{definition}[Dynamic $\delta$-AS Scheme Security]\label{def:DAS-security}

%     Let $\mathcal P$ be a correct dynamic Accountable Storage scheme consisting of the algorithms described in Definition~\ref{def:DAS}, $\mathcal A$ be a PPT adversary, and $\mathcal C$ be a challenger. Consider the following game between $\mathcal A$ and $\mathcal C$:
%     \begin{enumerate}
%         \item \emph{Initialization}. $\mathcal C$ generates $\{pk, sk\} \leftarrow KeyGen(1^\tau)$, sends $pk$ to $\mathcal A$ and keeps $sk$ secret. The adversary generates a set of blocks $B = \{b_1, ..., b_n\}$ and sends $B$ to the client.
%         \item \emph{Adaptive Chosen File Queries}. The adversary first specifies a set of blocks $B$ and provides them to $\mathcal C$. $\mathcal C$ then computes $state \leftarrow GenState(pk, B, \delta)$, which the client sends to the server. The server is allowed to issue any updates and can receive $state'$ from the client at each step. For a deletion, $\mathcal A$ must send the block to be removed, so that $\mathcal C$ can update their state. $\mathcal A$ will receive the response to that verification as well as the $\mathcal C$'s state after processing the update. 
%         \item \emph{Setup}. $\mathcal A$ decides on a sequence of operations. We reset the state, and $\mathcal A$ relates the updates to $\mathcal C$. $\mathcal C$ only makes updates to their local state if the updates are valid. 
%         \item \emph{Challenge}. $\mathcal C$ sends $chal \leftarrow GenChal(1^\tau)$ to $\mathcal A$ and requests a proof of accountability.
%         \item \emph{Forge}. $\mathcal A$ computes proof of accountability $\mathcal V$ and sends it to $\mathcal C$.
%     \end{enumerate}

%     $\mathcal A$ wins the game if $\mathcal L \leftarrow CheckAccountabilityProof(pk, sk, state, \mathcal V, chal)$ and either $|\mathcal L| > \delta$, $\mathcal L \not\subseteq B$, or $\mathcal C$ is unable to extract the remaining file blocks $B - \mathcal L$ from $\mathcal A$ using some PPT knowledge extractor $\varepsilon$ (i.e. $\mathcal A$ has successfully lied about preserving the remaining $B - \mathcal L$ blocks correctly). We say that $\mathcal P$ is secure if a PPT $\mathcal A$ wins the game with negligible probability.
% \end{definition}



==> sections/empirical.tex <==
\section{Empirical Results}\label{sec:empirical}

==> sections/peeling-strategy.tex <==
\section{Server Recovery}
\label{sec:peeling-iblt}
\ryuto{Does not have to be it's own section.}

tagSum is what is used to determine the purity of a cell.
\ryuto{Reference IBLT section of paper.}
Server cannot generate their own tags, thus cannot determine the purity of a
cell in the same way the client is able to.
However, the server can verify when a tag and block match.
Therefore, the server determines purity by checking if the tag and block match.
The server also checks their own tag set.
If they find it, and the block to match, everything is fine.
If they find the same tag, but a different block, then the block must have been
corrupted.
If they do not find the tag, then we assume we found a collision?
\ryuto{
Not sure if that's the best assumption to make,
but seems the most likely event.
}

